Deep Deformable 3D Caricatures with Learned Shape Control

A 3D caricature is an exaggerated 3D depiction of a human face. The goal of this paper is to model the variations of 3D caricatures in a compact parameter space so that we can provide a useful data-driven toolkit for handling 3D caricature deformations. To achieve the goal, we propose an MLP-based framework for building a deformable surface model, which takes a latent code and produces a 3D surface. In the framework, a SIREN MLP models a function that takes a 3D position on a fixed template surface and returns a 3D displacement vector for the input position. We create variations of 3D surfaces by learning a hypernetwork that takes a latent code and produces the parameters of the MLP. Once learned, our deformable model provides a nice editing space for 3D caricatures, supporting label-based semantic editing and point-handle-based deformation, both of which produce highly exaggerated and natural 3D caricature shapes. We also demonstrate other applications of our deformable model, such as automatic 3D caricature creation.

==> tex/macro.tex <==
\newcommand{\Eq}[1]  {Eq.~(\ref{eq:#1})}
\newcommand{\Eqs}[1] {Eqs.~(\ref{eq:#1})}
\newcommand{\Fig}[1] {Fig.~\ref{fig:#1}}
\newcommand{\Figs}[1]{Figs.~\ref{fig:#1}}
\newcommand{\Tbl}[1]  {Table~\ref{tbl:#1}}
\newcommand{\Tbls}[1] {Tables~\ref{tbl:#1}}
\newcommand{\Sec}[1] {Sec.~\ref{sec:#1}}
\newcommand{\Secs}[1] {Secs.~\ref{sec:#1}}
\newcommand{\Etal}   {{\textit{et~al.}}}
\newcommand{\Alg}[1] {Algorithm~\ref{alg:#1}}

\newcommand{\setone}[1] {\left\{ #1 \right\}} %
\newcommand{\settwo}[2] {\left\{ #1 \mid #2 \right\}} %

\newcommand{\todo}[1]{{\textcolor{blue}{TODO: #1}}}
\newcommand{\change}[1]{{\color{red}#1}}
\newcommand{\sean}[1]{{\textcolor{magenta}{sean: #1}}}
\newcommand{\yucheol}[1]{{\textcolor{magenta}{yucheol: #1}}}
\newcommand{\wonjong}[1]{{\textcolor{magenta}{wonjong: #1}}}
\renewcommand\tabularxcolumn[1]{m{#1}}
